Dual Prediction-Correction Methods for Linearly Constrained Time-Varying Convex Programs

Devising efficient algorithms to solve continuously-varying strongly convex optimization programs is key in many applications, from control systems to signal processing and machine learning. In this context, solving means to find and track the optimizer trajectory of the continuously-varying convex optimization program. Recently, a novel prediction-correction methodology has been put forward to set up iterative algorithms that sample the continuously-varying optimization program at discrete time steps and perform a limited amount of computations to correct their approximate optimizer with the new sampled problem and predict how the optimizer will change at the next time step. Prediction-correction algorithms have been shown to outperform more classical strategies, i.e., correction-only methods. Typically, prediction-correction methods have asymptotic tracking errors of the order of $h^2$, where $h$ is the sampling period, whereas classical strategies have order of $h$. Up to now, Prediction-correction algorithms have been developed in the primal space, both for unconstrained and simply constrained convex programs. In this paper, we show how to tackle linearly constrained continuously-varying problem by prediction-correction in the dual space and we prove similar asymptotic error bounds as their primal versions.

==> Approx.tex <==
% !TEX root = Dual_PC.tex
\section{Approximate time-derivative}\label{sec:approx}

In many practical scenarios the time derivative of the gradient of the cost function, e.g.,  $\nabla_{t\x}f$, is not directly available but has to be approximated or estimated in some ways. In this section, we show that similar results as Theorem~\ref{theo.main} hold even with an approximate time-derivative, if one employs a backward approximation as follows. 

Consider the mixed partial derivative at time $t_{k}$ using the gradient of the objective with respect to $\x$ at times $t_{k}$ and $t_{k-1}$, that is, the approximate partial mixed gradient $\tilde{\nabla}_{t\x}{f}_k$ as
%%%%
\begin{equation}\label{fobd}
\tilde{\nabla}_{t\x}f(\x_k; t_k) = \frac{1}{h} \left(\nabla_{\x}f(\x_k; t_k) - \nabla_{\x}f(\x_{k}; t_{k-1})\right), 
\end{equation}
%%%%
which is called a \textit{first-order backward finite difference} since it requires information of the first previous step for approximating the current mixed partial derivative. The error of this approximation is bounded on the order of $O(h)$~\cite{Quarteroni2000}, which may be improved by using the gradients and mixed partial derivative $\tilde{\nabla}_{t\x}f(\x_k; t_k)$  of more than one previous step, if needed\footnote{Approximation errors of the order of $O(h^2)$, $O(h^3)$, and $O(h^4)$ can be achieved, e.g., by the recursive method presented in~\cite{Lee1992}.}.
%

Substituting the partial mixed gradient $\nabla_{t\x} f(\x_k; t_k)$ in~\eqref{qp1} by its approximation $\tilde{\nabla}_{t\x}f(\x_k; t_k) $ in \eqref{fobd} leads to the {\it{approximate in time prediction step}}
%%%
\begin{equation}\label{appro_prediction}
\min_{\delta\x \in\mathbb{R}^n} \quad \frac{1}{2}\delta\x ^\transp \nabla_{\x\x} f(\x_k; t_{k})\delta\x +  \tilde{\nabla}_{t\x}f(\x_k; t_k)^\transp \delta\x, \quad \textrm{subject to } \A\delta\x = {\bf 0}.
\end{equation}
%%

\begin{corollary}\label{co:main}
The results of Theorem~\ref{theo.main} are still valid when using the approximate time-derivative in~\eqref{fobd} instead of the exact $\nabla_{t\x}f$, with an enlarged asymptotical error bound
\begin{subequations}\label{as_error_2}
\begin{align}
\limsup_{k\to\infty} \|{\blambda}_{k} - {\blambda}^*(t_{k})\| & = \frac{\varrho_{\textrm{C}}^{C}[\varrho_{\textrm{P}}^{P}(\Delta_2 \tilde{\Delta}_3 h + \Delta_2 C_0) + \Delta_2 \tilde{\Delta}_3 h]\,h + \frac{C_3}{2}\, h^2}{1 - \tau(h)},\\
\limsup_{k\to\infty} \|{\x}_{k} - {\x}^*(t_{k})\| &= \frac{\sigma_{\max}\varrho_{\textrm{C}}^{C-1} [\varrho_{\textrm{P}}^{P}(\Delta_2 (\tilde{\Delta}_3 h + \Delta_2 C_0) + \Delta_2 \tilde{\Delta}_3 h]\,h + \frac{C_3}{2}\, h^2}{[1 - \tau(h)] m},
\end{align}
\end{subequations}
where $\tilde{\Delta}_3 = \Delta_3+h \frac{C_3}{2}$.


\end{corollary}

{\bf PROOF.} Provided in the Appendix. \qed






==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

%strongly recommended
\numberwithin{theorem}{section}

% Declare title and authors, without \thanks
\newcommand{\TheTitle}{An Example Article} 
\newcommand{\TheAuthors}{D. Doe, P. T. Frank, and J. E. Smith}

% Sets running headers as well as PDF title and authors
\headers{\TheTitle}{\TheAuthors}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{{\TheTitle}\thanks{Submitted to the editors DATE.
\funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}}

% Authors: full names plus addresses.
\author{
  Dianne Doe\thanks{Imagination Corp., Chicago, IL
    (\email{ddoe@imag.com}, \url{http://www.imag.com/\string~ddoe/}).}
  \and
  Paul T. Frank\thanks{Department of Applied Mathematics, Fictional
    University, Boise, ID (\email{ptfrank@fictional.edu},
    \email{jesmith@fictional.edu}).}
  \and
  Jane E. Smith\footnotemark[3]
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> my_sections.tex <==
\usepackage{needspace}

% \nbsubsubsection{} provides a numbered subsection in bold without a line break. The section will contain at least three lines of text before a pagebreak
\newcommand{\nbsubsubsection}[1]{\needspace{1\baselineskip}\color{white}\subsubsection{#1}\vspace{-3\baselineskip}\color{black}\medskip{\noindent \bf \thesubsubsection. #1.}}

% \myparagraph provides a paragraph title in italics. 
\newcommand{\myparagraph}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}}

% \myindenetedparagraph provides an indented paragraph with title in italics.
\newcommand{\myindentedparagraph}[1]{\needspace{1\baselineskip}\medskip \hangindent=11pt \hangafter=0 \noindent{\it #1.}}

% \myparagraphtc provides a paragraph title in italics. It adds an enter to the table of contents
\newcommand{\myparagraphtc}[1]{\needspace{1\baselineskip}\medskip\noindent {\it #1.}\addcontentsline{toc}{subsubsection}{\qquad\qquad\quad#1}}


